OpeNPDN: A Neural-network-based Framework for Power Delivery Network Synthesis

Power delivery network (PDN) design is a nontrivial, time-intensive, and iterative task. Correct PDN design must account for considerations related to power bumps, currents, blockages, and signal congestion distribution patterns. This work proposes a machine learning-based methodology that employs a set of predefined PDN templates. At the floorplan stage, coarse estimates of current, congestion, macro/blockages, and C4 bump distributions are used to synthesize a grid for early design. At the placement stage, the grid is incrementally refined based on more accurate and fine-grained distributions of current and congestion. At each stage, a convolutional neural network (CNN) selects an appropriate PDN template for each region on the chip, building a safe-by-construction PDN that meets IR drop and electromigration (EM) specifications. The CNN is initially trained using a large synthetically-created dataset, following which transfer learning is leveraged to bridge the gap between real-circuit data (with a limited dataset size) and synthetically-generated data. On average, the optimization of the PDN frees thousands of routing tracks in congestion-critical regions, when compared to a globally uniform PDN, while staying within the IR drop and EM limits.

==> sec/related-work.tex <==
\ignore{
\section{Related Work}

\noindent
Several PDN optimization techniques that aim to build correct PDNs, while minimizing the PDN wiring area, have been proposed in the past few decades. These methods are primarily based on heuristics or optimization formulations, e.g., the works~\cite{Tan99, Wu04} proposed linear and non-linear programming-based optimization solutions respectively,~\cite{SHSN02} proposes a heuristic for signal congestion-aware PDN synthesis, and~\cite{SS06} proposes an algorithm which uses successive chip partitioning along with local PDN refinements to synthesize the PDN.  While all the above mentioned works use different optimization methods, they all involve calls to PDN analyzers at each iteration. Although PDN analysis has seen significant gains in efficiency through the use of based on multigrid methods~\cite{Kozhaya00}, hierarchical techniques~\cite{Zhao00, PengLi05}, or frequency domain approaches~\cite{Zhuang16}, these methods remain computationally prohibitive for full-chip PDN analysis, particularly if they are to be invoked repeatedly within the inner loop of an optimization scheme, as in~\cite{Tan99, Wu04, SHSN02, SS06}.  Moreover, most of these methods work with general power grid topologies that have no specific structure, which results in high analysis costs.  One exception is~\cite{SS06}, which uses the concept of locally regular, globally irregular grids, which resembles the concept of templates in this work, but this idea is only used for the top two metal layers in~\cite{SS06}. In contrast, we use a limited set of templates, and build templates that go across the entire interconnect stack.  

To overcome the slow heuristic-based nature of the PDN synthesis problem there have been a few recent efforts where ML has been applied to construct a routability and reliability-aware PDN.  The work in~\cite{Dey20} uses a multilayered perceptron to predict the width of the power stripes based on the current and its location as features. However, due to the unavailability of sufficient benchmarks, this work uses testcases that are small perturbations of the training set. Therefore, it is unclear if the multilayered perception generalizes across real test designs. The work in~\cite{Chang17} proposes an iterative method for PDN synthesis which calls a 
fast ML-based post-route wirelength and IR drop predictor under-the-hood.  However, the iterative nature of this ML-based method makes it slow. Both of these works construct uniform grids to meet 
worst-case IR drop. However, the PDNs are possibly overdesigned and may use more wiring resources than necessary. A more optimal irregular PDN could be customized to tune PDN density according to variations in current and congestion demands.

The work described in this paper builds upon OpeNPDN v1.0~\cite{OpeNPDNv1}, which had proposed a structured, yet flexible, approach to PDN design. The key to efficiency was the imposition of restrictions on the optimization search space by the use of technology-specific PDN templates, corresponding to DRC-correct PDN building blocks that vary in their metal layer utilizations. To employ these templates, the chip is tessellated into regions, and an ML approach is used to select one of the predefined PDN templates based on currents and congestion patterns in the region and its neighborhood. The templates are designed to guarantee connectivity when abutted, i.e., when any two different templates are assigned to adjacent regions. 

While OpeNPDN v1.0 was satisfactory under simplified design assumptions, the application of this method to more complex and realistic designs exposed several limitations that are rectified in this work.  While the earlier version used the spatial current distribution and the estimated signal routing congestion as features, for realistic designs, it was found that other features must also be incorporated. Notably:
\begin{itemize}
\item The distribution of C4 bump locations on a chip significantly impacts the voltage drop and current densities in a design.
\item Macro blocks, which are typically treated as blockages to standard cell power stripes, since they have presynthesized power grids within the blocks, can
impact the equivalent resistance between a region and C4 bumps as they effectively split the stripes in a PDN. \blueHL{The reader will ask: Why not hook up the macro power grid to the main power grid at the edges so that this is avoided? Good to answer this proactively -- assume this is not possible due to uncontrollable abutment requirements.}
\end{itemize}
We illustrate this through an example design whose current map, C4 bump, and blockage distributions are shown in Fig.~\ref{fig:macro-c4-influence}(a), we compare the IR drop of the chip with and without the blockages in Figs.~\ref{fig:macro-c4-influence}(b) and (c), respectively. The worst-case IR drop in the top-left corner of the chip is seen to be larger for the case with macro blockages, which create a longer indirect path between the top-left region of the chip and the C4 bumps. Therefore, the positions of the macros and C4 bumps are critical to IR drop and PDN synthesis.

\begin{figure}[thb]
\centering
\includegraphics[width=8.5cm]{fig/macro-c4-influence.pdf}
\caption{Influence of C4 bump locations, macros/PDN blockages on worst-case IR drop. (a) Current, C4 bump, and macro distributions and corresponding IR drop patterns (b) without and (c) with macros.}
\label{fig:macro-c4-influence}
\end{figure}

Due to the unavailability of a large set of benchmarks, OpeNPDNv1.0 trains the ML model using synthetically generated data and tests the model on RISC V cores. The key to transferability of this model depends on the diversity and realism of the synthetic data which is challenging to ensure as it requires the use of metrics that are difficult to define to evaluate the realism and diversity of the synthetic training set.
% \blueHL{Not clear why this is listed here. It seems that the features of v2.0 are in the li st below, and only the problems should be listed above, not the enhancements in v2.0.}
% \noindent
% The key limitations of ML-based prior art are listed below:
% \begin{itemize}
%     \item The power grids synthesized by the works in~\cite{Dey20, Chang17} are potentially sub-optimal (over-designed) as they {\it uniform} grids that constructed to meet worst-case IR drop across the chip.
%     \item The works in~\cite{OpeNPDNv1, Dey20, Chang17}C4 bumps and macro locations are key degrees of freedom which impact PDN synthesis.  which are key to PDN synthesis problem are unaccounted for~\cite{Dey20, OpeNPDNv1, Chang17}
%     \item Limited ML model transferability across designs due to unavailability of sufficient benchmarks for training and test which demands the use of synthetic benchmarks for training~\cite{OpeNPDNv1} or using perturbed training data as test~\cite{Dey20}
% \end{itemize}
}

\ignore{
\noindent
\underline{OpeNPDN v2.0} In this work, we overcome the above stated limitations of heuristic-based and prior ML-based PDN optimizers by the following key contributions:
\begin{enumerate}
    \item We propose an \textbf{ML-based} \textbf{fast} \textbf{correct-by-construction} PDN synthesis methodology to overcome its iterative nature. We show how ML enables (i) encapsulating the expensive PDN analysis step into a one-time training cost and (ii) rapid construction of a correct PDN during inference eliminating calls to expensive PDN analyzers.
    \item We define PDN templates to enable the ML-based methodology and synthesize an irregular PDN across the chip with piecewise regular pitches as against the uniform potentially over-designed  power grids.
    \item We account for currents, congestion, \textbf{C4 bumps, and macro distributions} as features to our ML methodology covering most degrees of freedom which impact correct static PDN synthesis.
    \item We employ \textbf{transfer learning} to train the CNN.  This helps overcome challenges with respect to limited number of available benchmarks in public domain and the lack of realism and diversity in the synthetic benchmarks in~\cite{OpeNPDNv1}. TL uses a large synthetically generated dataset as in~\cite{OpeNPDNv1} to pretrain the CNN and leverages TL and a handful of the real circuit data to train the CNN. The model once fully trained is reusable across any design implemented in the same technology.
\end{enumerate}
}


==> tbl/table_util.tex <==
\begin{table}[]
\caption{An example showing three templates $T_1, T_2, T_3$ showing their utilizations in M5 through M7.}
\label{tbl:util}
\centering
%\resizebox{1.00\columnwidth}{!}{%
{\scriptsize
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline
Metal layer &  Weights & \multicolumn{3}{c|}{PDN utilization} \\ \cline{3-5}
            &          & $T_1$    & $T_2$    & $T_3$ \\ \hline
M7          &  $w_7$   & $u_{71}$ & $u_{72}$ & $u_{73}$ \\ \hline
M6          &  $w_6$   & $u_{61}$ & $u_{62}$ & $u_{63}$ \\ \hline
M5          &  $w_5$   & $u_{51}$ & $u_{52}$ & $u_{53}$ \\ \hline
\end{tabular}
}
\end{table}

